IPC-GraspSim: Reducing the Sim2Real Gap for Parallel-Jaw Grasping with the Incremental Potential Contact Model

Accurately simulating whether an object will be lifted securely or dropped during grasping is a longstanding Sim2Real challenge. Soft compliant jaw tips are almost universally used with parallel-jaw robot grippers due to their ability to increase contact area and friction between the jaws and the object to be manipulated. However, interactions between the compliant surfaces and rigid objects are notoriously difficult to model. We introduce IPC-GraspSim, a novel grasp simulator that extends Incremental Potential Contact (IPC) - a highly accurate collision + deformation model developed in 2020 for computer graphics. IPC-GraspSim models both the dynamics and the deformation of compliant jaw tips to reduce Sim2Real gap for robot grasping. We evaluate IPC-GraspSim using a set of 2,000 physical grasps across 16 adversarial objects where analytic models perform poorly. In comparison to both analytic quasistatic contact models (soft point contact, REACH, 6DFC) and dynamic grasp simulators (Isaac Gym with FleX), results suggest IPC-GraspSim can predict robustness with higher precision and recall (F1 = 0.85). IPC-GraspSim increases F1 score by 0.03 to 0.20 over analytic baselines and 0.09 over Isaac Gym, at a cost of 8000x and 1.5x more compute time, respectively. All data, code, videos, and supplementary material are available at https://sites.google.com/berkeley.edu/ipcgraspsim.

==> includes/8-isaacgym-comp.tex <==
% % \begin{figure*}
% %     \centering
% %     \includegraphics[width=\textwidth]{figures/cube_3cm_ipc.png}
% %     \caption{IPC-GraspSim performance on cube}
% %     \label{fig:my_label}
% % \end{figure*}
% \begin{figure}
%     \centering
%     \includegraphics[width=0.5\textwidth]{figures/isaac-ipc-comp-example.png}
%     \caption{\todo{Isaac Gym - IPC comparison} In figure (cube comp), IPC success at ..., Isaac Gym miss at ...: we find that ... correctly simulates ..., but ... doesn't ... .}
%     \label{fig:my_label}
% \end{figure}
% \begin{figure}
%     \centering
%     \includegraphics[width=0.5\textwidth]{figures/gym-sim-comp.png}
%     \caption{Caption}
%     \label{fig:my_label}
% \end{figure}
% % Might be OK to just be a subsection.
% \section{In-depth Comparison with Isaac Gym}
% It is important to compare with Isaac gym because ... we choose this simulator to compare to because ... physics-based ... 
% \todo{insert further comparison here, cannot really put much stuff in because I haven't started on experiments for this section yet. However, we expect that Isaac gym would be better at accounting for grasps that leverage the rigid part of the gripper that IPC-GraspSim does not model. However, right now we hope that IPC will be better at modeling the friction and making sure the grasp works as expected.}


==> includes/x.notes.tex <==
% % Contact-GraspNet: Efficient 6-DoF Grasp Generation in Cluttered Scenes
% % https://arxiv.org/pdf/2103.14127.pdf
% % Noting "Model-based grasping" and "model-free grasping" - intro does a good job of doing pro/con of this
% % "The ability to grasp objects is one of the most fundamental capabilities required in robot manipulation tasks... involves reasoning about the 3D geometry and the physical properties... and also complex contact physics. It is studied in two main directions: model-based grasping... and model-free grasping... model-based grasping [predefines] a set of grasps [based on the prior knowledge about the object]."


% % % 1. Recap about field
% % Efficient and reliable robotic grasp planning is critical for fast object manipulation. Grasp quality calculation is run for each candidate grasp. Quality calculation needs to be completed in the order of milliseconds. Grasp models using simpler physics models are good for meeting both the time constraints while returning reasonable state estimation. They typically use quasistatic and rigid body models, which are simpler because the models have a lower degree of freedom. However, simple physical models fail to 1) consider post-grasp displacements that may cause objects to rotate out of place, and 2) utilize the compliant nature of deformable objects that allow for manipulation error.  % grasp changes mid-grasp from environment interaction including robot

% % Yet accurate simulators come at a cost; retrieving accurate and robust dynamics, friction, contact results take in the order of seconds to complete \cite{li2020incremental}, and even with the help of GPUs takes tens?hundreds? of milliseconds to calculate each dynamic grasp (Issac Gym dynamic rope estimate). Furthermore, simulators are very sensitive to parameter settings, and this is especially critical in a precise grap setting where everything matters. However, this does not change that considering dynamic and soft body models is critical for improving our estimated set of feasible grasps. 

% % % 2. Recap about problems in field + briefly about promising directions
% % % "customization requires flexible" - a survey on deep-learning grasp 
% % Other studies have tried to approach this by utilizing domain randomization during visual learning. Another study tried to learn when to trust the deformable model, in order to account for the inaccuracies \cite{mitrano2021learning}. An alternative approach to consider the physics is to approach robotic grasping from a deep learning perspective, training grasp planner models with datasets filled with synthetic grasps that consider the complex physics, such as ACRONYM \cite{eppner2020acronym}. However, this approach is difficult to extend as they fail to consider the difference in robot and gripper configurations. Regenerating the datasets is difficult since it requires lots of compute power. 

% % % 3. Introduce how this paper helps fix problem
% % % "HOPEFULLY we will allow for customize asdf"
% % % but what about non-parallel grippers?
% % % if this simulator can auto-tune then that would be amazing... 
% % This paper tackles this issue by ...?? Specifically, our experiments utilize a simulated parallel-jaw gripper padded with deformable material, and show that our simulator is highly accurate for the configurations they were tuned on. Then, we (try?) show how this model can be extended to other robot gripper configurations for novel grasps. (hard). 

% % \begin{figure}
% %     \centering
% %     \includegraphics[width=0.5\textwidth]{figures/example.png}
% %     \includegraphics[width=0.5\textwidth]{figures/example.png}
% %     \caption{Good IPC-sim modeling. Two difficult looking objects would be ideal. Not sure. But papers typically seem to have some figure of around this size with around this length of caption. }
% %     \label{fig:my_label}
% % \end{figure}

% % % 4. List contributions
% % Our primary contributions are:
% % \begin{enumerate}
% %     % Current work, working on validating it for IPC-net generation
% %     \item IPC-GraspSim: Grasping simulator extension from Incremental Potential Contact\cite{li2020incremental}
% %     % Planned item for when we have enough evidence 
% %     \item IPC-Net: Synthetic grasping data on over n simulated trials of grasping m single objects with IPC-GraspSim
% %     % "IPC-Tuner" sounds more like a maybe-item, but it would be nice since simulators are notorious for being sensitive. Something like auto-tune paper from bair the other time? Or OED stuff that DMODO is working on, extendable for this? 
% %     % Image segmentation?
% %     % \item IPC-Tuner: (online?) parameter tuning algorithm for IPC-GraspSim
% % \end{enumerate}
% % % we show that retraining state-of-the-art grasp planners... 
% % % maybe we can show that we see a consistent increase across many grasp planners + grippers to show 'extenability" and "generalizability"
% % We find that that GQ-CNN\cite{mahler2017dex} retrained with IPC-Net increases ... by ..., and decreases false positives by ... despite being trained only on synthetic data. 

% \textbf{Grasp simulators and grasp models}
% Grasp simulators typically branch into two different ways, either rigid or deformable materials. Rigid body grasp simulators are typically used in order to quickly evaluate grasps, in that case the simulator is not the main purpose, but typically used as a placeholder in order to leverage other features that are the "secret weapon" - such as utilizing depth images or generating grasps and pruning them down. In this case, the parameters are analytically calculated and chosen arbitrarily.

% On the other hand, the deformable grasp simulators typically focus on grasping deformable objects, if a focus on deformable materials, and the grippers are rigid. The contacts are typically limited to deformable-rigid contact. There are also grasp simulators for under-actuated compliant grippers, which also tend to have access to tactile sensors to use a closed-loop control scheme in order to refine its grasp. It is also noted in the compliant gripper paper that simulators are very sensitive to friction and closing forces, and found that deformable materials are difficult to tune for accuracy in all tested simulators. 

% A grasp model typically serves to measure the quality of a given grasp based on the environment, target object, and the robot grasp setting. A grasp model is typically provided antipodal grasps, and the grasps are evaluated based on some combination of friction, contact area, contact pressure, and resist-able wrench based on the contact. 

% \todo{Mention REACH and 6DFC as related work, since we talk about it in results as comparisons.}

% The success of a given grasp simulator is typically measured by if the given grasp matches the success rate in real, and the success of a given grasp model is typically measured by if a chosen grasp by the simulator will succeed in real. 

% \textbf{Sim2Real Learning for Object Manipulation}
% Due to the rise in machine learning and the increase in access to data, better sim2real by domain randomization, there has been an increase in learning physics-based simulators, and using the learned data to transfer to real. For object manipulation, binary objective success metrics can be used, checking if an object has been manipulated as expected. Most objects are assumed to be rigid. Sim2Real in objects are studied in a variety of different contexts, from rope and cloth manipulation to robotic grasping. Rope and cloth are typically studied to figure out if they reach the final desired configuration, while object grasping sim2real problems are typically studied to see if successful grasps in sim are also successful in sim. Another interesting one is learning parameters with differential evolution models. Typically, the learning is done iteratively in order to learn an applicable policy. Transfer learning is also common. Data augmentation is also done in clever ways, depending on the application. 
% \todo{List detailed work for sim2real / transfer learning / data augmentation brainstorming.}

% \textbf{Simulation of Deformable Materials}
% Simulation of deformable materials are challenging due to the high degree of freedom, and highly unpredictable due to friction. Self-intersections are also very common, as well as explosions due to the high parameter value sensitivity, causing catastrophic failures. Creating intersection-free contacts are inherently difficult due to the contact models typically employed. However, due to the high computational load, most work rely on simplified models as provided by pybullet and blender, where the simulation execution speeds are much more manageable and preferred by many current works. Particle-based physics models (DEM) are an alternative to the finite element approach, and are typically employed since they are easier to run in parallel on GPU, such as with Issac Gym. 

% More physically accurate, higher-fidelity finite element simulations are also very sensitive to parameter changes. However, commercial FEA software have typically tuned their parameters to the point that they will almost always return reliable values. They are typically used in engineering contexts, and take hours to run complex simulations. 

% The simulator performance is typically done by measuring their performance based on a given objective. There is a lot of successful work with co-dimensional bodies like strings and ropes, and cloths, where the body really exists in 1D or 2D space. In this case, they try to check, for instance, the keypoint location difference between sim and real. 
% % we are planning on having a video as well, and "drop test" is easier to show visually. 
% % Also, have a bigger section aboutwhy we chose IPC 
% \subsection{Background + Implementation}
% To generate our set of simulated grasps, Incremental Potential Contact\cite{li2020incremental} "IPC" work was used to build a robust grasp simulator. The simulator advertises its robustness and intersection-free solutions, which are critical for grasp simulations, since it allows for proper simulation of perturbations and prevents false positive grasp successes from objects intersecting and lodging themselves into the grippers. Furthermore, the work also finds the IPC simulator performs comparable to other commercial software with regards to \todo{fill here}. Also, IPC-GraspSim does not error out, which is better than others. \newline
% IPC-GraspSim extends IPC to simulate a piece-wise grasping motion, composed of:
% \begin{enumerate}
%     \item Close in until sufficient strain energy is reached in both deformable padding in the parallel jaw grippers
%     \item Stop closing motion, then lift gripper up with locked gripper position
%     % \item \todo{Angular rot. perturb?} % ~ to https://github.com/NVlabs/deformable_object_grasping
%     % \item \todo{Drop test?} 
% \end{enumerate}
% A simulated grasp is considered successful if both gripper jaws are in contact with the object at the end of simulation, and the object is lifted above ground. 

% \begin{figure}
%     \centering
%     \includegraphics[width=0.4\textwidth]{figures/rep_objs.png}
%     \caption{Representative objects: cat, pear, vase}
%     \label{fig:my_label}
% \end{figure}
% \begin{figure}
%     \centering
%     \includegraphics[width=0.3\textwidth]{figures/compliant_choices.png}
%     \caption{Square jaw, rounded jaw, actual jaw image.}
%     \label{fig:my_label}
% \end{figure}
% \subsection{Grasp Simulator Tuning}
% Physics-based simulators often come with a myriad of parameters and are notoriously hard to tune due to parameter sensitivity, and friction is also difficult to model correctly. Furthermore, silicon rubber is a nonlinear elastic material, so it is crucial to find the correct material constants to model the material given the grasping range. \newline
% For this section, we choose four demonstrative objects from our physical dataset (cube, cat, pear, vase) for parameter tuning, as they contain a variety of flat, sharp, and round surfaces in their corresponding grasps. Grasps for other objects are then used with the same parameter for simulator performance testing. \todo{Quantitative why the objects are representative objs}. \newline
% We currently limit ourselves to manual tuning. We manually perform a grid search of varying gripper properties: geometry, Young's modulus, and friction coefficient when interacting with the target object. Then, we choose the set of parameters that performs the best on average across the demonstrative objects. 
